MoSculp: Interactive Visualization of Shape and Time

We present a system that allows users to visualize complex human motion via 3D motion sculptures---a representation that conveys the 3D structure swept by a human body as it moves through space. Given an input video, our system computes the motion sculptures and provides a user interface for rendering it in different styles, including the options to insert the sculpture back into the original video, render it in a synthetic scene or physically print it. To provide this end-to-end workflow, we introduce an algorithm that estimates that human's 3D geometry over time from a set of 2D images and develop a 3D-aware image-based rendering approach that embeds the sculpture back into the scene. By automating the process, our system takes motion sculpture creation out of the realm of professional artists, and makes it applicable to a wide range of existing video material. By providing viewers with 3D information, motion sculptures reveal space-time motion information that is difficult to perceive with the naked eye, and allow viewers to interpret how different parts of the object interact over time. We validate the effectiveness of this approach with user studies, finding that our motion sculpture visualizations are significantly more informative about motion than existing stroboscopic and space-time visualization methods.

==> figText/img_userstudy.tex <==
 \begin{figure*}[t!]
 	\includegraphics[width=\linewidth]{fig/img_userstudy.pdf}
 	%\vspace{-15pt}
	\caption{The images for our user studies. From left to right: our motion sculptures, stroboscopic photography, and shape-time photography~\protect\cite{freeman:shapetime}.}
 	%\vspace{-10pt}
	\label{fig:img_userstudy}
 \end{figure*}


==> text/abstract.tex <==
\begin{abstract}

We present a system that allows users to visualize complex human motion via 3D \emph{\summarynames}--a representation that conveys the 3D structure swept by a human body as it moves through space. Given an input video, our system computes the \summaryname and provides a user interface for rendering it in different styles, including the options to insert the sculpture back into the original video, render it in a synthetic scene or physically print it.

To provide this end-to-end workflow, we introduce an algorithm that estimates that human's 3D geometry over time from a set of 2D images and develop a 3D-aware image-based rendering approach that embeds the sculpture back into the scene. By automating the process, our system takes \summaryname creation out of the realm of professional artists, and makes it applicable to a wide range of existing video material.

By providing viewers with 3D information, \summarynames reveal space-time motion information that is difficult to perceive with the naked eye, and allow viewers to interpret how different parts of the object interact over time. We validate the effectiveness of this approach with user studies, finding that our \summaryname visualizations are significantly more informative about motion than existing stroboscopic and space-time visualization methods. 


%Motion sculptures, due to their 3D nature, reveal space-time
%information that is difficult to detect by the naked eye, and they allow  viewers to interpret how different parts of the object interact over
%time. We validated this in a user study and found that 78
%percent of participants were able to better perceive fine details
%about complex motions from our visualization over existing
%stroboscopic or space-time visualization approaches.

%We present a system for visualizing complex human motion via 3D \emph{motion sculptures}---a representation that conveys
%the 3D structure swept by the human's body as it moves through space. With only a standard RGB video from the user, our system  computes a motion-sculpture by estimating the object's 3D geometry over time, and then provide the user with an interactive interface to render the motion sculpture under different styles, either on top of the original video, into a synthetic scene, or 3D print it. 

%To accomplish this end-to-end workflow, we developed an algorithm that first automates the 3D motion sculpture construction process from a set of 2D images, and then places the motion sculpture back into the scene. For this, we developed a 3D-aware image based rendering approach that preserves the depth ordering.
%By automating the process, our system takes motion sculpture creation out of the realm of professional artists, and makes it accessible to novice users and applicable to a wide range of existing video material.

 %In addition, the image information is also used to reconstruct the texture on the motion sculpture. 

%Motion sculptures, due to their 3D nature, reveal space-time information that is difficult to detect by the naked eye, and they allow a viewer to interpret how different parts an object interact over time. We validated this in a user study and found that 78 percent of participants could perceive better fine information about complex motions from our visualization over existing stroboscopic or space-time visualization approaches. 

%The reason for this is that our motion sculptures reveal space-time information that participants were otherwise not able to detect, and also allowed participants to interpret how different parts of the object interact over time.



% NEW ABSTRACT
% We present a system that allows users to visualize complex human motion via 3D \emph{motion sculptures}---a representation that conveys the 3D structure swept by a human's body as it moves through space. Our system automates the process of estimating motion sculptures from input videos, and the process of virtually inserting them back into the source video. For this, we introduce a method for estimating human 3D structure from videos that is well-suited to constructing motion sculptures, as well as a 3D-aware image-based rendering approach that preserves the scene's depth ordering. Our system is applicable to a wide range of existing videos, and it provides users a variety of ways to choose how the motion sculpture is rendered, and to correct errors in the pose estimation process. By automating the process, our system takes motion sculpture creation out of the realm of professional artists, and makes it accessible to novice users. 


% Motion sculptures reveal space-time motion information that is difficult to perceive with the naked eye, and it allows viewers to interpret how different parts of the object interact over time. We validate the effectiveness of this approach with user studies, finding that our motion sculpture visualizations are significantly more informative about motion than existing stroboscopic and space-time visualization methods. 


%Given an input video, our system computes the motion-sculpture by estimating the object's 3D geometry over time. In addition, our system provides the user with an interactive interface to render the motion sculpture under different styles, either on top of the original video, into a synthetic scene, or 3D print it. 

%To accomplish this end-to-end workflow, we developed an algorithm that first automates the 3D motion sculpture construction process from a set of 2D images, and then places the motion sculpture back into the scene. For this, we developed a 3D-aware image based rendering approach that preserves the depth ordering. By automating the process, our system takes motion sculpture creation out of the realm of professional artists, and makes it accessible to novice users and applicable to a wide range of existing video material.

 %In addition, the image information is also used to reconstruct the texture on the motion sculpture. 
%We validated this in a user study and found that 78 percent of participants were able to better perceive fine details about complex motions from our visualization over existing stroboscopic or space-time visualization approaches. 

%The reason for this is that our motion sculptures reveal space-time information that participants were otherwise not able to detect, and also allowed participants to interpret how different parts of the object interact over time.


\end{abstract}

